Autonomous Learning for Face Recognition in the Wild via Ambient Wireless Cues

Facial recognition is a key enabling component for emerging Internet of Things (IoT) services such as smart homes or responsive offices. Through the use of deep neural networks, facial recognition has achieved excellent performance. However, this is only possibly when trained with hundreds of images of each user in different viewing and lighting conditions. Clearly, this level of effort in enrolment and labelling is impossible for wide-spread deployment and adoption. Inspired by the fact that most people carry smart wireless devices with them, e.g. smartphones, we propose to use this wireless identifier as a supervisory label. This allows us to curate a dataset of facial images that are unique to a certain domain e.g. a set of people in a particular office. This custom corpus can then be used to finetune existing pre-trained models e.g. FaceNet. However, due to the vagaries of wireless propagation in buildings, the supervisory labels are noisy and weak.We propose a novel technique, AutoTune, which learns and refines the association between a face and wireless identifier over time, by increasing the inter-cluster separation and minimizing the intra-cluster distance. Through extensive experiments with multiple users on two sites, we demonstrate the ability of AutoTune to design an environment-specific, continually evolving facial recognition system with entirely no user effort.

==> section/preliminaries.tex <==
%!TEX root = ../autotune.tex
\section{Preliminaries} % (fold)
\label{sec:preliminaries}

\begin{figure}[t]\centering
\includegraphics[width=\columnwidth]{fig/event_def.pdf}  
\caption{An illustrative example of \emph{events} and showing their linked face and device \emph{observations}. An \emph{event} is uniquely determined by spatial-temporal attributes and its participants. An event is also linked with two types of observations. The face observation are images cropped from surveillance videos and the device observation are sniffed MAC address of participants' devices.}
\label{fig:event_def}
\end{figure}

\subsection{Key Terms} % (fold)
\label{sub:key_terms}
In this section, we introduce some key terms and background that pave the way for \sect\ref{sec:autotune_solution}. 

\noindent \textbf{Event}:
As we will soon discuss in the next section, a key concept in {\sysname} is that of an \emph{event}. An event $e \in E$ is the setting in which people interact with each other in a specific part of the environment for a given time interval. It is uniquely identified by three attributes: effective timeslot, location, and participants. Fig.~\ref{fig:event_def} demonstrates a few examples of events. As we can see, an instance of an event might be a meeting in a conference room, exercise in a gym, or a lunch in the canteen. The spatio-temporal attributes of an event, i.e., timeslot and location, can either be obtained by side channel information (e.g. calendar), or for simplicity, they can be assumed to be fixed size cubes. However, the participants of an event, especially if it happens in a public space, are difficult to directly obtain. Details about how we create events in real-word experiments will be introduced in \sect\ref{ssub:event_duration}.

% \begin{definition}{(\textbf{Event})}
% An event $e \in E$ is the setting that subjects interact with entities in an environment for a time interval. It is uniquely identified by three attributes: effective timeslot, happening location, and involved (subject) identities. 
% \end{definition}
\noindent \textbf{observations}:
A smart camera and a WiFi sniffer are assumed to sense the identities in an environment. With the rapid development of camera systems and increasing deployment of WiFi access points, our assumption is practical. With these two sensor modalities, two types of observations can be attached to an event: i) cropped face images detected by the cameras, and ii) device observations (MAC addresses) which give weak user attendance or presence information through WiFi sniffing. Fig.~\ref{fig:event_def} illustrates the relationship between identity observations and events through examples.

\noindent \textbf{Pre-trained Model}:
A pre-trained model is used to transform the face images into discriminative features or representations, thereby aiding accurate clustering or classification. In this work, a deep neural network (DNN) for discriminative face representation is trained by a model provider, e.g., Facebook or Google, who are able to access a large number of annotated face images. This model needs to be fine-tuned by smart-cameras in a particular space or environment, e.g., images acquired from an office or home. Note that our formulation does not require access to the images used for pre-training, just the weights and architecture of the pre-trained network model. 

\subsection{Challenges and Objectives} % (fold)
\label{sub:challenges_and_objectives}
{\sysname} is motived by the fact that, neither of the above sensor observations can \emph{directly} provide \emph{accurate} identity information. Face images are strong biometrics, but they cannot directly convey identity information without external labels i.e. a recognition model is needed to transfer biometrics to actual identity. The pre-trained model is no exception here. Given the mapping between MAC address and user identity, device observations are able to provide unique and direct identity information. In practice, the mapping between a MAC address to a user is easy to get for cameras in smart spaces. In order to authenticate legitimate WiFi users, say Eduroam \footnote{https://en.wikipedia.org/wiki/Eduroam}, device MAC addresses and user account information are bound together. However, device observations are usually noisy because a detected MAC address does not necessarily indicate that the device owner is co-located. Therefore, the objectives of {\sysname} are two-fold: i) automatically label face images that have noisy observations; and ii) reliably adapt the pre-trained model to recognize the faces of users in new environments.
% subsection notations (end)

==> section/problem.tex <==
%!TEX root = ../autotune.tex
\section{Problem Statement} % (fold)
\label{sec:problem_statement}

\begin{figure}[t]\centering
\includegraphics[width=\columnwidth]{fig/event_def.pdf}  
\caption{An illustrative example of \emph{event} and its face and WiFi \emph{observations}. \chris{will complete the caption}}
\label{fig:intuition}
\end{figure}


\subsection{Preliminaries} % (fold)
\label{sub:preliminaries}
\subsubsection{Background} % (fold)
\label{ssub:background}
Initially, a deep neural network (DNN) for discriminative face representation is trained by a model provider, e.g., Facebook or Google, who are able to access a large amount of annotated face images. We refer to this pre-trained model as the \emph{donor model} and it needs to be fine-tuned by smart-cameras in a particular space or environment, e.g., images acquired from an office or home. Note that our formulation does not require access to the images used for pre-training, just the weights and architecture of the pre-trained model. In addition to the donor model, a smart camera environment also possesses two types of data: i) cropped face images detected by the cameras, and ii) device observations (MAC addresses) which give weak presence information through WiFi sniffing. 

\subsubsection{Challenges and Objectives} % (fold)
\label{ssub:challenges_and_objectives}
Face images are strong biometrics, but they cannot directly convey identity information without external labels i.e. a recognition model is needed to transfer biometrics to actual identity. Given the mapping between MAC address and user identity, device observations are able to provide unique and direct identity information. In practice, the mapping between a MAC address to a user is easy to get for cameras in smart spaces. In order to authenticate legitimate WiFi users, say Eduroam \footnote{https://en.wikipedia.org/wiki/Eduroam}, device MAC addresses and user account information are bound together. However, device observations are usually noisy because a detected MAC address does not necessarily indicate that the device owner is co-located. Therefore, the objectives of AutoTune are two-fold: i) automatically label face images that have noisy observations; and ii) reliably adapt the donor model to recognize the faces of users in new environments.

\subsubsection{Key Terms} % (fold)
\label{ssub:key_terms}
 We assume a collection of $n$ images $\{x_i \in X\}_{i=1}^n$ are collected by one or more smart cameras, which contains the cropped face images of users. These will have wide variability e.g. different views, poses, scales and illumination. Let $\{l_j \in L\}_{j=1}^m$ be a set of $m$ WiFi MAC addresses, i.e., $m$ people of interest (POI) to recognize. The instance-level labels $\{y_i^{\tau} \in L\}_{i=1}^n$ match the identities to the face images $\{x_i \in X\}_{i=1}^n$ at iteration $\tau$. With the updated model $f_{\theta}^{\tau}$, a face image $x_i$ is transformed to a feature representation $\{z_i^{\tau} \in Z\}_{i=1}^n$. After $T$ iterations, the resultant model is denoted as $f_{\theta}^T$. 

\subsection{Problem Formulation} % (fold)
\label{sub:problem_formulation}
AutoTune adapts the donor model by iteratively minimizing two losses in tandem: i) the face representation loss $\mathcal{L}_R$ and ii) the identity association loss $\mathcal{L}_A$, which will now be discussed in turn.
\subsubsection{Representation Loss} % (fold)
\label{ssub:representation_loss}
The representation loss $\mathcal{L}_R$ reflects how discriminative the learned face features are. Strong discrimination bears two properties: inter-class dispersion and intra-class compactness. Inter-class dispersion pushes face images of different subjects away from one another and the intra-class compactness pulls the face images of the same subject together. Both of these steps are critical to face recognition. At iteration $\tau$, given the current labels $y_i^{\tau}$ for the $i$th face image $x_i$ and the transformed features $z_i^{\tau} = f_{\theta}^{\tau}(x_i)$, the representation loss $\mathcal{L}_R$ is determined by a composition of softmax loss and center loss:

\begin{equation}
	\begin{split}
		\mathcal{L}_R &= \mathcal{L}_{softmax} + \mathcal{L}_{center} \\
				      &= \underbrace{\sum_{i}-log(\frac{e^{W_{y_i^{\tau}}^Tz_i^{\tau} + b_{y_i^{\tau}}}}{\sum_{j=1}^{m}e^{W_{l_j}^Tz_i^{\tau} + b_{l_j}}})}_\text{softmax loss} + \underbrace{\sum_{i}\frac{\lambda}{2} ||z_i^{\tau} - c_{y_i^{\tau}}||^2}_\text{center loss}
	\end{split}
	\label{equ:model_loss}
\end{equation}
where $W$ and $b$ are the weights and bias parameters in the last fully connected layer of the pre-trained model. The center loss $\mathcal{L}_{center}$ explicitly enhances the intra-class compactness while the inter-class dispersion is implicitly strengthened by the softmax loss $\mathcal{L}_{softmax}$ \cite{wen2016discriminative}. $\lambda$ is a hyper-parameter that balances the above sub-losses. 

\subsubsection{Association Loss} % (fold)
\label{ssub:association_loss}
The association loss $\mathcal{L}_A$ measures how accurately the device ID is assigned to the face images. At iteration $\tau$, the ID assignment is a linear programming problem:
\begin{equation}
	\begin{split}
		& \mathcal{L}_A = \sum_{ij} a_{ij}^{\tau} \varepsilon_{ij}^{\tau} \\
		 \sum_{1 \leq j \leq m} & a_{ij}^{\tau} = 1, \quad \forall i \in \{1, \ldots, n\}
	\end{split}
	\label{equ:loss}
\end{equation}
where $a_{ij}^{\tau}$ is a binary variable that is set to $1$ if the face image is assigned to identity label $j$, and $0$ otherwise. The parameter is $\varepsilon_{ij}^{\tau}$ is the cost of such an assignment and will be discussed in detail in \sect\ref{ssub:fine_grained_id_association}. As we can see, the association loss is also constrained to guarantee that exactly one identity label is given to an image, but not vice versa. Through minimizing the the association loss $\mathcal{L}_A$, the label $y_i^{\tau+1}$ of an image can be derived by the optimal assignment of $a_{ij}^{\tau}$ at iteration $\tau$.                                                                                                                                    
% At a high level, the optimization of the total losses goes as follows. At the first iteration $\tau=0$, the face images $X$ are grouped into clusters $G^{0}$, based on the similarity of their transformed features $Z^{0}$ using the donor model $f_{\theta}^{0}$. The clusters of face images are then associated with the device MAC addresses, to achieve the minimum association costs of $\mathcal{L}_A$. The cost $\varepsilon_{ij}$ of association will be shortly introduced in the next section. Images in the same cluster then share the same assigned identity label $Y^0$. The labels assigned in the association step, will be leveraged to fine-tune the representation model $f_{\theta}^{0}$. Above association and fine-tuning steps completes one iteration. The optimization keep perform such iterations, until converges. The model $f_{\theta}^{T}$ derived in the last iteration (t=T) is taken as the final model adapted to the new environment. 




==> section/solution.tex <==
%!TEX root = ../autotune.tex
\section{AutoTune Solution} % (fold)
\label{sec:autotune_solution}
\begin{figure}[t]\centering
\includegraphics[width=0.99\columnwidth]{fig/autotune_arch_v2.pdf}  
\caption{Workflow of {\sysname}. {\sysname} consists of 5 steps i) Event segmentation ii) Cross-Modality clustering iii) Cluster Labeling iv) Visual Model Update v) User Attendance Update. {\sysname} sequentially repeats the above five steps until the changes in the user attendance model are negligible.}
\label{fig:architecture}
\end{figure}

% \subsection{Event Segmentation} % (fold)
% \label{ssub:event_segmentation}

% As defined in \sect\ref{ssub:event}, an event is denoted as $e$. We assume a collection of $n$ images $\{x_i \in X\}_{i=1}^n$ are collected by one or more smart cameras, which contain the cropped face images of users. These will have wide variability, e.g., different views, poses, scales and illumination. Let $\{l_j \in L\}_{j=1}^m$ be a set of $m$ WiFi MAC addresses, i.e., $m$ people of interest (POI) to recognize. 

% Assuming after data collection, we have images $\{x_i \in X\}_{i=1}^n$ spanning multiple events, e.g., over the period of several days. {\sysname} segments images into $|E|$ subsets, namely the number of events. An image subset $\{x_{e_k, i} \in X_{e_k}\}$ in event $e_k$ is determined by the captured time and camera location. For instance, any images captured during the timeslot of event $e_k$, e.g, 14:00-15:00 on the 1st of May, by cameras in a particular room, are put into the image subset $X_{e_k}$. All the images in the same subset share the same event index. It is worth noting that one subject could have multiple face images in $\{x_{e_k, i} \in X_{e_k}\}$, e.g., captured at different lighting conditions or viewing angles. On the other hand, by inspecting the sniffed MAC addresses, we can also maintain an $m$-dimensional attendance observation vector $I_{e_k}^{\tau}$ for each event. $I_{e_k}^{\tau}[j]$ which is set to $1$ only if the user $j$'s MAC address $l_j \in L$ is detected in the event $e_k$. We refer readers to Fig.~\ref{fig:event_def} to see the examples of such event attachments. Due to the uncertain nature of WiFi sensing, the initial attendance observation $I_{e_k}^{\tau}$ is noisy and should be iteratively updated. These event attachments build \textit{coarse-grained} correlations between a set of face images and a set of device IDs, through their shared event $e_k$. However, at this stage the fine-grained mapping between an image $x_{e_k, i}$ and a MAC address $l_{e_k, j}$ is unknown. Note that, in the following sections, we use the superscript $\tau$ to denote the $\tau$-th iteration of those variables which will be updated in {\sysname}.

% \begin{figure}[t]\centering
% \includegraphics[width=0.75\columnwidth]{fig/i-clustering.pdf}  
% \caption{Cross-modality clustering. The final similarity is jointly determined by attendance assistance derived from event logs and similarity of features transformed via $f_{\theta}$, see Equ.~\ref{equ:id-ass_sim}. Detailed explanations can be found in \sect\ref{ssub:identity_assisted_clustering}.} 
% \label{fig:i-clustering}
% \end{figure}

\subsection{Cross-modality Clustering} % (fold)
\label{ssub:identity_assisted_clustering}
Before assigning fine-grained ID labels, {\sysname} needs to cluster images across events. Unlike conventional clustering that merely depends on the feature similarity, {\sysname} merges face images \textit{across events} into a cluster (potentially belonging to the same subject) by incorporating attendance information as well. Recall that the attendance observation vector $I_{e_k}^{\tau}$ already reveals the identities of subjects (in the form of MAC addresses) in the event $e_k$, and the captured images $X_{e_k}$ may contain the faces of these subjects. Despite the noise in observations, the overlapped subjects in different events can be employed as a prior that guides the image clustering. For example, if there are no shared MAC addresses sniffed in two events, then it is very likely that the face images captured in these two events should lie in different clusters. 

Formally, the likelihood that two cross-event face images $x_{e_k, i}$ and $x_{e_p, j}$ belong to the same subject is conditioned on two factors: i) the similarity of their feature representation between $z_{e_k, i}^{\tau}$ and $z_{e_p, j}^{\tau}$; and ii) the overlap ratio between the attendance observations in their corresponding events. The resulted joint similarity is a log likelihood $log(\mathbf{Pr}(y_{e_k, i}^{\tau} = y_{e_p, j}^{\tau}))$ defined as follows:

\begin{equation}
\begin{split}
	\mathbf{Pr}(y_{e_k, i}^{\tau} = y_{e_p, j}^{\tau}) 
	& \propto \frac{exp(\beta * |I_{e_k}^\tau \otimes I_{e_p}^\tau|)}{exp(\beta * |I_{e_k}^\tau \oplus I_{e_p}^\tau|)} * exp(-D(z_{e_k, i}^{\tau}, z_{e_p, j}^{\tau})) \\
	log(\mathbf{Pr}(y_{e_k, i}^{\tau} = y_{e_p, j}^{\tau})) & \propto \beta * \underbrace{(|I_{e_k}^\tau \otimes I_{e_p}^\tau| - |I_{e_k}^\tau \oplus I_{e_p}^\tau|)}_\text{attendance assistance} - \underbrace{D(z_{e_k, i}^{\tau}, z_{e_p, j}^{\tau})}_\text{feature distance}
	\label{equ:id-ass_sim}
\end{split}
\end{equation}

Here $\otimes$ and $\oplus$ are element-wise AND and OR, and $|\cdot|$ here is the $L^1$-norm. $z$ is the features transformed by the face representation model and $D$ is a distance measure between face features. $\beta$, \chris{analogous to the regularization parameter in composite loss functions,} is a hyper-parameter that controls the contributions of the attendance assistance and feature similarity. Fig.~\ref{fig:i-clustering} demonstrates how the joint similarity between two cross-event images is determined. The above derivation is inspired by the Jaccard coefficients, with the difference lying in the log function. The rationale behind the term $|I_{e_k} \oplus I_{e_p}|$ is that the more different subjects attending events, the more uncertain that any two images drawn across these events will point to the same subject. In contrast, when the intersection $|I_{e_k} \otimes I_{e_p}|$ is significant enough, the chance that these two images point to the same subject will become higher. \chris{Equ.~\ref{equ:id-ass_sim} can also be explained from a Bayesian perspective. The attendance similarity of two events can serve as a prior that two cross-event images belong to the same subject and the feature similarity can be seen as the likelihood. Together they determine the posterior probability that two cross-event images fall into the same cluster.} Based on the above joint similarity, images across events are grouped into $g$ clusters. We will soon discuss how to determine $g$ based on the complete set of MAC addresses $\{l_j \in L\}_{j=1}^m$ in \sect\ref{ssub:voting}.

\begin{figure}[t]\centering
\includegraphics[width=0.99\columnwidth]{fig/event_vector.pdf}  
\caption{Event vectors of an image cluster and device ID. The $k$th element of the vector $V_{G_i}[k]$ is set to $1$ only it contains images attached with the event $e_k$. The event vector $V_{l_j}$ of the device ID $l_j$ is similarly developed. See \sect\ref{sub:cross_modality_labeling} for more details.} 
\label{fig:event_vector}
\end{figure}

\subsection{Cluster Labeling} % (fold)
\label{sub:cross_modality_labeling}
\subsubsection{Fine-grained ID Association} % (fold)
\label{ssub:fine_grained_id_association}
After clustering, an image cluster is linked with multiple events that are associated with its member images. We introduce an event vector $V_{G_i}^{\tau}$ for an image cluster $G_i$, with $V_{G_i}^{\tau}[k]$ that is set to 1 only if it contains images attached with the event $e_k$. The length of the event vector is determined by the number of events $|E|$. Fig.~\ref{fig:event_vector} shows an example of how an event vector is developed. Similarly, for a device ID $l_j$, its corresponding event vector $V_{l_j}^{\tau}$ can be determined by inspecting its occurrences in all user attendance observations. $V_{l_j}^{\tau}[k]$ is set to $1$ only if the device ID (MAC address) $l_j$ is detected in the event $e_k$. \chris{The intuition behind ID association is that the device and the face image cluster of the same subject should share the most consistent attendance pattern in events, reflected by the similarity of their event vectors. Based on this intuition, {\sysname} assigns cluster $G_i$ with device IDs based on the matching level of their event vectors.} Formally, a matching problem of bipartite graph can be formulated as follows:
\begin{equation}
	\begin{split}
		& \mathcal{L}_A = \sum_{ij} a_{ij}^{\tau} (V_{G_i}^{\tau} - V_{l_j}^{\tau})^2 \\
		 & \sum_{1 \leq j \leq m}  a_{ij}^{\tau} = 1, \quad \forall i \in \{1, \ldots, g\}
	\end{split}
\end{equation}
where the solution of the binary variable $a_{ij}^{\tau}$ assigns a device ID to a cluster, and the images in a cluster are labeled by the same assigned ID. We note that when $m<g$, {\sysname} adds dummy nodes to create the complete bipartite graph. Then the complete bipartite graph problem can be solved by the Hungarian algorithm \cite{jonker1986improving}.

\subsubsection{\chris{Probabilistic Labeling via Soft Voting}} % (fold)
\label{ssub:voting}
We now obtain the instance-level ID association. However, in practice, the number of clusters $g$ can vary due to the captured face images outside the POI, e.g., face images of short-term visitors. The choice of $g$ has a significant impact on the performance of clustering \cite{fraley1998many} which could further affect the following fine-tuning performance. To include the non-POI, the number of clusters $g$ should be greater than the number of POI $m$, but the exact number of $g$ is impossible to know beforehand. To bypass this issue, we set the cluster number $g$, from $2*m$ to $5*m$ and run the clustering (\sect\ref{ssub:identity_assisted_clustering}) and association (\sect\ref{ssub:fine_grained_id_association}) for multiple rounds. {\sysname} is robust to extra clusters of non-POI, when $g$ is greater than $m$. Although there are some unused clusters of non-POI after clustering, the association step will sieve them and only choose the most consistent $m$ clusters with the event logs of $m$ device IDs. Lastly, for every image, its assigned ID is finalized by decision voting on the individual association results computed with different $g$, ranging from $2*m$ to $5*m$.

Typically, a majority voting procedure would give a hard ID label for an image and use these $<$Image, ID$>$ pairs as training data to update the face representation model. However, due to the noise in device presence observations and errors in clustering, there will be mis-labeling in the training data that may confuse the model update. To account for the uncertainty of ID assignment, we adopt soft labels for voting. More specifically, instead of voting for the most likely ID $y_i^{\tau}$ for an image $x_i$, we introduce a normalized vector $m$-dimension $\mathbf{y}_{i}^{\tau}$. \chris{Specifically, every image is associated with all POI and its associated soft label is derived by the votes for the subjects divided by the total number of votes. In this way, the soft label of each image is a valid probability distribution that sums up to 1.} For instance, $\mathbf{y}_{i}^{\tau}[j]=0.4$ means that there are $40\%$ associations assigning the ID $j$ to the image $i$. Moreover, the soft labeled data $<x_i, \mathbf{y}_{i}^{\tau}>$ is compatible with the computation of cross-entropy. \chris{  Besides coping the uncertain number of non-POI, soft voting can actually handle the feature uncertainty issue of outliers. Outliers of POI refer to those images belongs to a POI but very dissimilar to the majority. Those images can significantly confuse the clustering process. We observed that, with a proper clustering algorithm (i.e., agglomerative clustering in our choice), outlier images will form separate small clusters but they will not be chosen in our follow-up association step. This is because that the number of devices ID $m$ is always less than the number of clusters ($[2*m, 5*m]$), and only those images clusters with the most consistent event attendances are associated. The small clusters of outlier images often have scatted attendance vector and will be ignored in association. Therefore, soft voting with varying number of clusters can reinforce the core images of POI by giving large probability and assigns outlier images with very small probability.
} 

% \begin{figure}[t!]
% 	\centering
% 	\begin{subfigure}{0.32\textwidth}
% 	\includegraphics[width=\linewidth]{fig/eval/wifi_cm/nobar/no_start.pdf}
% 	\caption{Initial WiFi Attendance \emph{Obser.} } 
% 	\end{subfigure}\hspace*{\fill}
% 	\begin{subfigure}{0.32\textwidth}
% 	\includegraphics[width=\linewidth]{fig/eval/wifi_cm/nobar/no_cycle_8.pdf}
% 	\caption{Attendance \emph{Obser.} after 1st iter.} 
% 	\end{subfigure}\hspace*{\fill}
% 	\begin{subfigure}{0.36\textwidth}
% 	\includegraphics[width=\linewidth]{fig/eval/wifi_cm/bar/bar_cycle_15.pdf}
% 	\caption{Attendance \emph{Obser.} after 3rd iter.}
% 	\end{subfigure}

% 	\medskip
% 	\centering
% 	\begin{subfigure}{0.32\textwidth}
% 	\includegraphics[width=\linewidth]{fig/eval/wifi_cm/nobar/no_diff.pdf}
% 	\caption{Initial Attendance \emph{Errors}} 
% 	\end{subfigure}\hspace*{\fill}
% 	\begin{subfigure}{0.32\textwidth}
% 	\includegraphics[width=\linewidth]{fig/eval/wifi_cm/nobar/no_diff_cycle_6.pdf}
% 	\caption{Attendance \emph{Errors} after 1st iter.}
% 	\end{subfigure}\hspace*{\fill}
% 	\begin{subfigure}{0.36\textwidth}
% 	\includegraphics[width=\linewidth]{fig/eval/wifi_cm/bar/bar_diff_cycle_15.pdf}
% 	\caption{Attendance \emph{Errors} after 3rd iter.}
% 	\end{subfigure}

% \caption{An example of user attendance update (\sect\ref{ssub:id_update}) in {\sysname}, a 15-subject subset of $20$ events. \textbf{Top}: Attendance observations in events; \textbf{Bottom}: (absolute) errors of attendance observations in events. It can be seen that the IDs in events are gradually corrected as the model updates in {\sysname}.} \label{fig:id_update}
% \end{figure}

\subsection{Visual Model Update} % (fold)
\label{sub:model_update}
We are now in a position to introduce the model update in {\sysname}. By taking the labeled data as inputs, the face representation model $f_{\theta}^{\tau}$ updates its weights and biases $\theta$ to $f_{\theta}^{\tau+1}$. 

\subsubsection{Discriminative Face Representation} % (fold)
\label{ssub:discriminative_face_repre}
Face representation learning optimizes a representation loss $\mathcal{L}_R$ to force the learnt features as discriminative as possible. Strong discrimination bears two properties: inter-class dispersion and intra-class compactness. Inter-class dispersion pushes face images of different subjects away from one another and the intra-class compactness pulls the face images of the same subject together. Both of the properties are critical to face recognition. At iteration $\tau$, given the current labels $y_i^{\tau}$ for the $i$th face image $x_i$ and the transformed features $z_i^{\tau} = f_{\theta}^{\tau}(x_i)$, the representation loss $\mathcal{L}_R$ is determined by a composition of softmax loss and center loss:
\begin{equation}
	\begin{split}
		\mathcal{L}_R &= \mathcal{L}_{softmax} + \mathcal{L}_{center} \\
				      &= \underbrace{\sum_{i}-log(\frac{e^{W_{y_i^{\tau}}^Tz_i^{\tau} + b_{y_i^{\tau}}}}{\sum_{j=1}^{m}e^{W_{l_j}^Tz_i^{\tau} + b_{l_j}}})}_\text{softmax loss} + \underbrace{\sum_{i}\frac{\lambda}{2} ||z_i^{\tau} - c_{y_i^{\tau}}||^2}_\text{center loss}
	\end{split}
	\label{equ:model_loss}
\end{equation}
where $W$ and $b$ are the weights and bias parameters in the last fully connected layer of the pre-trained model. The center loss $\mathcal{L}_{center}$ explicitly enhances the intra-class compactness while the inter-class dispersion is implicitly strengthened by the softmax loss $\mathcal{L}_{softmax}$ \cite{wen2016discriminative}. $\lambda$ is a hyper-parameter that balances the above sub-losses. 

\subsubsection{Fuzzy Center Loss} % (fold)
\label{ssub:fuzzy_center_loss}
The center loss $\mathcal{L}_{center}$ in Equ.~\ref{equ:model_loss} is shown to be helpful to enhance the intra-class compactness \cite{wen2016discriminative}. However, we cannot directly adopt it for fine-tuning as computing the centers requires explicit labels (see Equ.~\ref{equ:model_loss}) of images, but the association steps above only provide probabilistic ones through soft labels. To solve this, we propose a new loss called \emph{stochastic center loss} $\mathcal{L}_{stoc}$ to replace the center loss. Similar to the core idea of fuzzy clustering \cite{xie1991validity}, we allow each face image to belong to more than one subject. In fact, the membership grades indicating the degree to which an image belongs to each subject can be directly retrieved from the soft labels and the stochastic center $\mathbf{o}_k^{\tau}$ is given as:

\begin{equation}
	\mathbf{o}_k^{\tau} = \frac{\sum_i^{n}\mathbf{z}_i^{\tau} * y_{i,k}^{\tau}}{\sum_i^{n} y_{i,k}^{\tau}}
	\label{equ:fuzzy_center}
\end{equation}
The fuzzifier $\eta$ is a hyper-parameter that determines the level of cluster fuzziness. A large $\eta$ results in smaller membership values and hence, fuzzier clusters. This gives the stochastic center loss as follows:
\begin{equation}
\mathcal{L}_{stoc} = \sum_{i}\sum_{k} \mathbf{y}_{i}^{\tau}[k]*||z_i^{\tau} - \mathbf{o}_k^{\tau}||^2
\end{equation}

\subsubsection{Fine-tuning} % (fold)
\label{ssub:fine_tuning}
We leave the softmax loss $\mathcal{L}_{softmax}$ the same as in Equ.~\ref{equ:model_loss}, because the soft labels are compatible with the computation of cross-entropy. The new representation loss to minimize is:
\begin{equation}
	\mathcal{L}_R = \mathcal{L}_{softmax} + \mathcal{L}_{stoc}
\end{equation}
{\sysname} updates the model parameters $\theta^{\tau}$ to $\theta^{\tau+1}$ based on the gradients of $\nabla_{\theta}\mathcal{L}_R$, which are calculated via back prorogation of errors. Compared with the dataset used for pre-training, which is usually in the order of millions \cite{cao2017vggface2}, the data used for fine-tuning is much smaller (several thousands). The mis-match between the small training data and the complex model architecture could result in overfitting. To prevent overfitting, we use the dropout mechanism in training, which is widely adopted to avoid overfitting \cite{lecun2015deep}. Meanwhile, as observed in \cite{hinton2015distilling,reed2014training}, the soft label itself can play the role of a regularizer, and make the trained model robust to noise and reduce overfitting.

\subsection{User Attendance Update} % (fold)
\label{ssub:id_update}
The device presence observations by WiFi sniffing are noisy because the WiFi signal of a device is opportunistic and people do not carry/use theirs devices all the time. Based on the results of the cluster labelling step introduce in \sect\ref{sub:cross_modality_labeling}, we have the opportunity to update our belief on which users attended each event. 

The update mechanism is as follows: Each image is associated with a user probability vector, whose elements denote the probability that the image correspondences to a particular user. By averaging the user probability vectors of all images that have been drawn from the same event ${e_k}$, and normalizing the result, we can estimate the user attendance of this event. The elements of the resulting user attendance vector $\hat{I}_{e_k}$ denote the probabilities of different users attending event ${e_k}$. 

We can now use $\hat{I}_{e_k}$ as a correction to update our previous wifi attendance vector $I_{e_k}^{\tau}$  as follows:

\begin{equation}
	I^{\tau+1}_{e_k} = I^{\tau}_{e_k} - \beta \cdot (I^{\tau}_{e_k} - \hat{I}_{e_k})
\end{equation}
where $\beta$ is a pre-defined parameter that controls the ID update rate. In principle, a large update rate will speed up the convergence rate, at the risk of missing the optima.

\begin{figure*}[t!]
	\centering
	\begin{subfigure}{0.2\textwidth}
	\includegraphics[width=\linewidth]{fig/eval/tsne/50/2018-04-02-114759_tnse.pdf}
	\caption{Pre-trained Model} \label{fig:tnse_pretrain}
	\end{subfigure}\hspace*{\fill}
	\begin{subfigure}{0.2\textwidth}
	\includegraphics[width=\linewidth]{fig/eval/tsne/50/2018-05-05-13-23-29_tnse.pdf}
	\caption{1st iteration}
	\end{subfigure}\hspace*{\fill}
	\centering
	\begin{subfigure}{0.2\textwidth}
	\includegraphics[width=\linewidth]{fig/eval/tsne/50/2018-05-06-06-04-50_tnse.pdf}
	\caption{2nd iteration} 
	\end{subfigure}\hspace*{\fill}
	\begin{subfigure}{0.2\textwidth}
	\includegraphics[width=\linewidth]{fig/eval/tsne/50/2018-05-05-15-14-23_tnse.pdf}
	\caption{3rd iteration} 
	\end{subfigure}

\caption{An example of visual model update (\sect\ref{sub:model_update}) in {\sysname} with a six subject subset. Note that the pre-trained model in Fig.~\ref{fig:tnse_pretrain} has a narrow convex hull (black lines), clusters are dispersed and there is misclassification. After the first iteration, clusters become more distinct and span more of the embedding space. Over time, clusters become more compact and move further away from each other, leading to purer clustering results.} \label{fig:model_update}
\end{figure*}

{\sysname} sequentially repeats the above steps of clustering, labelling and model updates, until the changes in the user attendance model are negligible. Algorithm.~\ref{alg:autotune} summarizes the workflow.

\begin{algorithm}[h] 
\KwIn{pre-trained model $f_{\theta}^{0}$, WiFi sniffed attendance observations $I^{0}$, images $X$, number of POI $m$, threshold $\xi$}
\KwOut{adapted model $f_{\theta}^{\ast}$, corrected attendance observations $I^{\ast}$, soft image labels $Y^{\ast}$} 
\kwInit{Segment attendance observations $I^0$ and images $X$ into subsets $I^0_{e_k}$ and $X_{e_k}$ based on events $E$ \Comment{\sect\ref{ssub:event_segmentation}}} 
$\tau=0$ \\
\While{$\sqrt{\frac{1}{|E|}\sum_{k=1}^{|E|}||I^{(\tau)}_{e_k} - I^{(\tau-1)}_{e_k}||^2} > \xi$}{
	$Z^\tau = f_{\theta}^{\tau}(X)$ \Comment{feature transformation}\\
	\For{$g \leftarrow m$ to $3*m$}{
	 	$G^\tau \leftarrow$ \texttt{cross\_modality\_clustering}($Z^\tau$, $I^\tau$, g) \Comment{\sect\ref{ssub:identity_assisted_clustering}}\; 
	 	$A^\tau_g \leftarrow$ \texttt{ID\_association}($G^\tau$, $I^\tau$) \Comment{\sect\ref{ssub:fine_grained_id_association}}\; 
	}
	$Y^{\tau} \leftarrow$ \texttt{voting}($A^\tau$) \Comment{\sect\ref{ssub:voting}}\;
 	$c^{\tau} \leftarrow$ \texttt{fuzzy\_center}($Y^{\tau}$, $Z^\tau$) \Comment{\sect\ref{ssub:fuzzy_center_loss}}\; 
 	$f_\theta^{\tau+1} \leftarrow$ \texttt{visual\_model\_update}($Y^\tau$, $c^\tau$, $f_\theta^{\tau}$, X) \Comment{\sect\ref{ssub:fine_tuning}} \;
 	$I^{\tau+1} \leftarrow$ \texttt{user\_attendance\_update}($Y^{\tau}$, $I^{\tau}$) \Comment{\sect\ref{ssub:id_update}} \;
  $\tau \leftarrow \tau + 1$
 }
% \nl \bf Pass\;
    \caption{{\bf {\sysname}} \label{alg:autotune}}

\end{algorithm}


